A Survey of Local Differential Privacy and Its Variants

The introduction and advancements in Local Differential Privacy (LDP) variants have become a cornerstone in addressing the privacy concerns associated with the vast data produced by smart devices, which forms the foundation for data-driven decision-making in crowdsensing. While harnessing the power of these immense data sets can offer valuable insights, it simultaneously poses significant privacy risks for the users involved. LDP, a distinguished privacy model with a decentralized architecture, stands out for its capability to offer robust privacy assurances for individual users during data collection and analysis. The essence of LDP is its method of locally perturbing each user's data on the client-side before transmission to the server-side, safeguarding against potential privacy breaches at both ends. This article offers an in-depth exploration of LDP, emphasizing its models, its myriad variants, and the foundational structure of LDP algorithms.

==> other.tex <==
\section{Local Differential Privacy, Properties and Mechanisms}

In this section, we study LDP and its properties, and LDP based mechanisms. We start from the definition of LDP.


\textbf{Definition 1} ($\varepsilon$-Local Differential Privacy ($\varepsilon$-LDP) . \\
A randomized mechanism $M$ satisfies $\varepsilon$-LDP if and only if for any pairs of input values $v$, $v'$ in the domain of $M$, and for any possible output $y \in Y$, it holds
\begin{equation}
P[M(v) = y] \leq e^{\varepsilon} \cdot P[M(v') = y],
\end{equation}
where $P[\cdot]$ denotes probability and $\varepsilon$ is the privacy budget. A smaller $\varepsilon$ means stronger privacy protection, and vice versa.


The basic properties of LDP includes the followings:



\textbf{Composition:} 
Given two mechanisms $M_1$ and $M_2$ that provide $\varepsilon_1$-LDP and $\varepsilon_2$-LDP respectively, their sequential composition provides $(\varepsilon_1 + \varepsilon_2)$-LDP.
\begin{equation}
M(v) = (M_1(v), M_2(v)) \implies M \text{ is } (\varepsilon_1 + \varepsilon_2) \text{-LDP}
\end{equation}

\textbf{Post-processing:} 
Any function applied to the output of an $\varepsilon$-LDP mechanism retains the $\varepsilon$-LDP guarantee.
\begin{equation}
\text{If } M(v) \text{ is } \varepsilon\text{-LDP, then } f(M(v)) \text{ is also } \varepsilon\text{-LDP} .
\end{equation}

\textbf{Robustness to Side Information:} 
LDP guarantees hold even if an adversary has access to auxiliary or side information.

\textbf{Utility-Privacy Tradeoff:} 
Generally, a lower value of $\varepsilon$ implies stronger privacy but might result in reduced utility of the perturbed data.

\textbf{Independence of Background Knowledge:}
The privacy guarantees of LDP mechanisms are designed to hold regardless of any background knowledge an adversary might have.


Next, we study mechanisms that satisfies LDP: 

\textbf{Randomize Response}

The Randomized Response Mechanism is a simple yet effective approach to achieve LDP. It's particularly used for binary data, i.e., when a user's data item is either $0$ or $1$. The mechanism operates as follows:

\begin{enumerate}

\item With probability $\frac{1}{2}$, the user truthfully answers a question.
\item With probability $\frac{1}{2}$, the user randomly answers the question.

\end{enumerate}

Mathematically, given a user's true data item $v \in \{0, 1\}$, the mechanism outputs $v$ with probability $\frac{1}{2}$ and outputs $1 - v$ (i.e., the opposite of $v$) with probability $\frac{1}{2}$.

The probability mass function (pmf) is given by:
\begin{align}
P[M(v) = 1] &= \frac{1}{2} v + \frac{1}{2} (1 - v) = \frac{1}{2} \\
P[M(v) = 0] &= \frac{1}{2} (1 - v) + \frac{1}{2} v = \frac{1}{2}
\end{align}

This mechanism ensures $\varepsilon$-LDP with $\varepsilon = \ln(2)$.



\textbf{Laplace Mechanism}

The Laplace Mechanism adds noise drawn from the Laplace distribution to the true value of the data. For LDP, this mechanism can be adjusted as:

Given a data item \( v \), the mechanism outputs:
\[ M(v) = v + \text{Lap}(\frac{\Delta f}{\varepsilon}) \]
where \( \Delta f \) is the sensitivity of the function \( f \) and \( \text{Lap}(\cdot) \) represents the Laplace distribution.

\textbf{Gaussian Mechanism}

Similar to the Laplace Mechanism, the Gaussian Mechanism adds noise but from the Gaussian distribution:

Given a data item \( v \), the mechanism outputs:
\[ M(v) = v + \mathcal{N}(0, \sigma^2) \]
where \( \sigma^2 \) determines the amount of noise based on the desired \( \varepsilon \) and function sensitivity \( \Delta f \).

\textbf{Exponential Mechanism}

The Exponential Mechanism selects an output based on a scoring function and weights outputs with the exponential of their score. Given a set of possible outputs \( R \), a data item \( v \), and a scoring function \( q(v, r) \), the probability of selecting output \( r \) is proportional to:
\[ \exp\left(\frac{\varepsilon q(v, r)}{2\Delta q}\right) \]
where \( \Delta q \) is the sensitivity of \( q \).

\textbf{Perturbed Histogram Mechanism}

For a set of items, instead of perturbing each item, this mechanism perturbs the histogram of the data items. Given a data item set \( V \), the mechanism constructs a histogram \( H \) and then outputs:
\[ M(H) = H + \text{Lap}(\frac{\Delta H}{\varepsilon}) \]
where \( \Delta H \) is the sensitivity of the histogram construction.

Observe that each mechanism's efficacy is closely tied to the sensitivity of the query, denoted as \( \Delta f \). In the realm of Local Differential Privacy (LDP), this sensitivity can often grow significantly, especially when the input domain is vast. The larger the sensitivity, the more noise needs to be introduced by the mechanism to ensure the desired privacy level. This can lead to significant distortion in the data, compromising its utility.

Furthermore, as the input support size increases, maintaining the desired privacy guarantee becomes a challenge. Noise calibrated to a high sensitivity can sometimes overshadow the actual data, rendering the results almost meaningless or leading to misinterpretations.

The consequence of this is a pronounced tradeoff between utility and privacy. Achieving stronger privacy often means accepting reduced accuracy and utility in the results, and vice versa. For applications that require high precision, this can be problematic. It implies that while these mechanisms provide a robust privacy guarantee in theory, their practical applicability can be constrained, especially in scenarios where fine-grained insights from data are crucial. 

Hence, while the promise of LDP is enticing, its real-world implementation requires careful consideration of the utility-privacy balance, pushing researchers to seek more efficient mechanisms or modified privacy models to better cater to practical needs.

\section{Advanced LDP mechanisms }

As we mentioned in the introduction, to improve the utility-privacy tradeoff provided by LDP, there are typically two manners. One is to design dedicated mechanism or advanced protocols. The other is to relax the definition of LDP to enhance the data utility. In this section, we summarized several advanced LDP algorithms, aiming to improve the general utility-privacy tradeoff.

\section{LDP variants and mechanisms}

\subsection{Variants and Mechanisms of LDP}

\subsubsection{\( (\varepsilon, \delta) \)-LDP}
Drawing parallels with how \( (\varepsilon, \delta) \)-DP \cite{50} extends \( \varepsilon \)-DP, \( (\varepsilon, \delta) \)-LDP (sometimes termed as approximate LDP) serves as a more flexible counterpart to \( \varepsilon \)-LDP (or pure LDP). 

\begin{defi}[Approximate Local Differential Privacy]
A randomized process \( M \) complies with \( (\varepsilon, \delta) \)-LDP if, for all input pairs \( v \) and \( v' \) within \( M \)'s domain and any probable output \( y \in Y \), the following holds:
\[ P[M(v) = y] \leq e^{\varepsilon} \cdot P[M(v') = y] + \delta. \]
Here, \( \delta \) is customarily a small value.
\end{defi}

In essence, \( (\varepsilon, \delta) \)-LDP implies that \( M \) achieves \( \varepsilon \)-LDP with a likelihood not less than \( 1-\delta \). If \( \delta = 0 \), \( (\varepsilon, \delta) \)-LDP converges to \( \varepsilon \)-LDP.

\subsubsection{BLENDER Model}
BLENDER \cite{52}, a fusion of global DP and LDP, optimizes data utility while retaining privacy. It classifies users based on their trust in the aggregator into two categories: the opt-in group and clients. BLENDER enhances utility by balancing data from both. Its privacy measure mirrors that of \( (\varepsilon, \delta) \)-DP \cite{50}.

\subsubsection{Local d-privacy}
Originally tailored for location privacy with global DP, Geo-indistinguishability \cite{53} uses the data's geographical distance. Alvim et al. \cite{54} argued for metric-based LDP's advantages in specific contexts.

\begin{defi}[Local d-Privacy]
A randomized function \( M \) adheres to local d-privacy if, for any input pairs \( v \) and \( v' \) and any output \( y \in Y \), the subsequent relation is met:
\[ P[M(v) = y] \leq e^{\varepsilon \cdot d(v, v')} \cdot P[M(v') = y], \]
where \( d(., .) \) designates a distance metric.
\end{defi}

This model adjusts privacy depending on data distance, augmenting utility for datasets like location or smart meter consumption that are sensitive to distance.

\subsubsection{CLDP}
Recognizing LDP's diminished utility with fewer users, Gursoy et al. \cite{56} introduced the metric-based model condensed local differential privacy (CLDP).

\begin{defi}[\( \alpha \)-CLDP]
For all input pairs \( v \) and \( v' \) in \( M \)'s domain and any potential output \( y \in Y \), a randomized function \( M \) satisfies \( \alpha \)-CLDP if:
\[ P[M(v) = y] \leq e^{\alpha \cdot d(v, v')} \cdot P[M(v') = y], \]
where \( \alpha > 0 \).
\end{defi}

In CLDP, a decline in \( \alpha \) compensates for a growth in distance \( d \). Gursoy et al. employed an Exponential Mechanism variant to devise protocols, particularly benefitting scenarios with limited users.

\subsubsection{PLDP}
PLDP \cite{7,57} offers user-specific privacy levels. Here, users can modify their privacy settings, denoted by \( \varepsilon \).

\begin{defi}[\( \varepsilon \)-PLDP]
For a user \( U \), and all input pairs \( v \) and \( v' \) in \( M \)'s domain and any potential output \( y \in Y \), a randomized function \( M \) meets \( \varepsilon_U \)-PLDP if:
\[ P[M(v) = y] \leq e^{\varepsilon_U} \cdot P[M(v') = y]. \]
\end{defi}

Approaches like the personalized count estimation protocol and advanced combination strategy cater to users with varying privacy inclinations.





